Bandits for BMO Functions

We study the bandit problem where the underlying expected reward is a Bounded Mean Oscillation (BMO) function. BMO functions are allowed to be discontinuous and unbounded, and are useful in modeling signals with infinities in the do-main. We develop a toolset for BMO bandits, and provide an algorithm that can achieve poly-log $\delta$-regret -- a regret measured against an arm that is optimal after removing a $\delta$-sized portion of the arm space.

==> tex/discussion.tex <==


\section{Discussion}

In this section, we discussion some properties of our algorithm, and compare it to related previous algorithms. 

\subsection{Breaking `` Needle In A Haystack''}

Compare to previous works for bandits in metric spaces, our algorithm generalizes to beyond continuous function. In addition, with proper choices of $\alpha$ and $\beta$, the $0$-regret of Bandit-BMO can grow much slower than the regret of Zooming bandit. 
%has a weaker dependence on dimensionality at the same time. 
We are able to achieve this by using the $\epsilon$-regret, and utilizing some basic measure properties. Recall that in Zooming bandit, a lower bound on the regret for bandit problem is derived using the ``needle-in-a-haystack'' argument, which was first used in \citep{}. In this argument, we construct a hard problem instance, where one arm is slightly better than the rest of the arms, and all other arms are equally good. 

This argument, however, is forbidden by the definition of $0$-regret, since in this case, the good arm is of measure zero, and will be ignored by definition. 

In both real-world setting and analysis of metric measure spaces, it is standard to apply almost everywhere arguments and thus ignore sets of measure zero. 

%In a metric measure space, ignoring a set of measure zero is reasonable 

%While our algorithm serves as the first bandit algorithm for BMO functions, it has . Perhaps the most related works are the Zooming bandit algorithm and the HOO algorithm, which also run by maintaining partitions of the space. 
%The regret bounds however, are not directly comparable, since of course $ \epsilon $-regret and plain regret are not comparable. Yet, when allowing a small tolerance of non-optimality, our . This . 

\subsection{Generalizability of Enclidean Space}

Throughout the paper, we have constrained our discussion to the Euclidean space. However, this setting can be made as general as spaces considered in previous works (e.g. Zooming bandit \citep{}), with a proper scaling of the metric. 

To see this, we first review the definitions of doubling spaces and Zooming dimension. 

\begin{definition}
 \label{def:doubling}
      A metric space $(X,d)$ is said to be geometrically doubling (or simply doubling) if any ball $B(x,r) \subset X$ can be covered by at most $N$ balls $B \left( x_i, \frac{r}{2} \right)$ for some $N < \infty$ and some centers $x_1, \cdots, x_N$. We call $N$ the doubling number of the space $(X,d)$, and call $\log_2 N$ the doubling dimension of the space $(X,d)$. 
\end{definition}

As suggested by the definition of doubling space, there are metric spaces where there exists a ball that cannot be covered by finitely many balls of half its radius. In fact, the functional space $  $ is not doubling. To see this, we first argue that doubling dimension is no smaller than the Hausdorff dimension \citep{}, and from classic texts \cite{}, we know that this space has infinite Hausdorff dimension. 

\begin{definition}
 \label{def:zooming-dimension}
 	Let $(X,d)$ be a metric space, and let $f$ be the payoff function of a problem instance. For any $\delta>0$, let $X (\delta, f) := \{ x \in X, f^* - f(x) < \delta \}$, where $f^* := \max_{x^\prime \in X} f (x^\prime)$. 
 	The Zooming dimension of payoff function $f$ in $(X,d)$ is the smallest $ N $, such that there exists $N > 0$, such that 
 	
\end{definition}

From this definition, we can see that in order for the Zooming dimension to be finite for any payoff function, we need the underlying metric space $(X,d)$ to be a doubling space. Otherwise, we can find a ball $B_0$ that cannot be covered by finitely many balls of half its radius, and then find a payoff function $f_0$ and a number $\delta_0$ such that $X (\delta_0, f_0) = B_0$. 

In fact, as asserted by the Assouad Embedding Theorem, any doubling space can be embedded in to the Euclidean space with proper scaling of the metric. Below we quote a fairly recent version of the Assouad Embedding Theorem \citep{}, for a precise statement. For more details on the Assouad Embedding Theorem, we refer the readers to \citep{} and references therein. 

\begin{theorem}[Assouad Embedding Theorem]
	
\end{theorem}

Indeed, hypercubes in the Euclidean space is itself a very interesting subject, and is sometimes referred to as Dyadic Systems \citep{}, and shall be interesting in learning. 

%\subsection{Dyadic of Enclidean Space}









==> tex/exp-new.tex <==
% \vspace{-10pt}
\section{Empirical Study}
% \vspace{-8pt}
\label{sec:exp} 

% Since the TreeUCB algorithm imposes only a set of mild constraints on tree formation, we use greedy decision tree training to fit the reward function, instead of controlling only the region diameters and the partition cardinality. 


% \vspace{-8pt}
\subsection{Synthetic Data}
% \vspace{-5pt}
Although the setting of Bandit-BMO is much more general, we study its empirical performance on synthetic continuous functions. 
In particular, 
% \textcolor{red}{grammar and punctuation are messed up on this sentence} 
we compare the performance of Bandit-BMO against the HOO algorithm and the Zooming Bandit Algorithm. 
% We also compare the performance of CTUCB against the Contextual Zooming Bandit Algorithm and the CCKL-UCB algorithm. Here, we set $\eta = 2$ for the tree fitting rule, we set $M = 0.1$ and $C = 0.001$ for TUCB. For the other algorithms, the coefficient for the exploration term are all 1. In particular for HOO, we set $v_1 = 0.1, \rho = 0.1$ (see Algorithm 1 in \cite{bubeck2011x} for details about their $v$ and $\rho$ in HOO's setting). We use the Himmelblau's function and the Goldstein function 
% for the simulated experiments. 
The synthetic test functions are two-dimensional. 
% In the experiments for contextual algorithms, 1) we use one input dimension of the test function as the context, and this dimension is randomly sampled at each round; 2) we let the algorithm choose a point (an arm) from the other dimension. The details for this functions are deferred to Appendix \ref{app:exp}. 

As shown in Figure \ref{fig:synthetic-function}, Bandit-BMO algorithm outperforms benchmark algorithms on synthetic data. 
% The performance gain is from the fact TreeUCB is \textit{adaptively learning} the partition, instead of only controlling the global partition. 

\begin{figure}[h!]
% \label{fig:synthetic-function}
\centering
\vspace{-0.4cm}
% \subfloat[Goldstein]{\includegraphics[width = 0.4 \textwidth]{./figures/compare_non_contextual_goldstein.png} } \\
\subfloat[Himmelblau]{ \includegraphics[width = 0.4 \textwidth]{./figures/compare_non_contextual_himmelblau.png} }
% \subfloat[Goldstein]{ \includegraphics[width = 0.225 \textwidth]{./figures/compare_contextual_goldstein} }
% \subfloat[Himmelblau]{ \includegraphics[width = 0.225 \textwidth]{./figures/compare_contextual_himmelblau} }
\caption{Each line plot is averaged over 10 runs, and the corresponding shaded area indicates the standard deviation. All methods use 1 as exploration parameter. Bandit-BMO corresponds to Bandit-BMO with $\alpha = 0.6$, $ \beta = 1.2$. 
% ($\eta$ is the parameter mentioned at the beginning of Section \ref{sec:exp}).  
\label{fig:synthetic-function} }
\vspace{-0.6cm}
\end{figure}


% % \vspace{-8pt}
% \subsection{Neural Network Tuning}
% \label{sec:tune-nn}
% % \vspace{-5pt}
% One application of stochastic bandit algorithms is zeroth order optimization. In this section, we apply TUCB to tuning neural networks. In this setting, we treat the hyperparameter configurations (e.g. learning rate, network architecture) as arms, and use validation accuracy as reward. The task is to select a hyperparameter configuration and train the network to observe the validation accuracies, and locate the best hyperparameter configuration as soon as possible. 

% \begin{figure}%
% \centering
% \includegraphics[scale = 0.3]{./figures/legend.png} \\
% \subfloat[MLP for MNIST]{\includegraphics[scale = 0.3]{./figures/MNIST_non_contextual.png} \label{fig:tune-nn-mnist}}
% \subfloat[CNN for SVHN]{ \includegraphics[scale = 0.3]{./figures/SVHN_non_contextual.png} \label{fig:tune-nn-svhn}}
% \subfloat[AlexNet-CNN for CIFAR-10]{ \includegraphics[scale = 0.3]{./figures/CIFAR_non_contextual} \label{fig:tune-nn-cifar}}
% \caption{Performance of TUCB against benchmark methods in tuning neural networks \label{fig:tune-nn} }
% \vspace{-8pt}
% \end{figure}

% In Figure \ref{fig:tune-nn}, the results shows that TUCB is competitive with benchmark methods in the task of tuning neural networks. See Appendix \ref{app:exp-nn} for details about hyperparameter space for this experiments. 



==> tex/theory-heavy-tail.tex <==

\section{Heavy Tail} \label{sec:zooming-theory}

This part uses the same machinery from Bubeck et al 2012. 
We assume that the noise has bounded $(1+\epsilon)$-th moment: there exists a constant $u$, such that for any arm $a$,
\begin{align}
	\mathbb{E}[ | \mathpzc{E}_a |^{1 + \epsilon} ] \le u. 
\end{align}

We use the truncated mean trick for heavy-tail noise. For a number $\delta > 0$, we define
\begin{align}
	m_t^{tr} (l) := 
	\begin{cases}
    \frac{\sum_{i = 1 }^{ t - 1 } Y_i \mathbbm{1}_{[A_i \in l ]} \mathbbm{1}_{[|Y_i| \le B_i ]} }{ n_{t} (l) } , 
    \text{ if }  n_{t}(l) > 0;  \label{eq:average}
    \\
    0, \quad \text{otherwise}. 
    \end{cases}  
\end{align}
where $n_t$ is defined as in (\ref{eq:count}), and $B_i := \left(  \frac{ \left( 2^{3 + 2\epsilon}  \Psi^{1 + \epsilon} + 2^{1 + \epsilon} u   \right)i }{\log \left( 1/ \delta \right) } \right)^{\frac{1}{1 + \epsilon}} $. 


%Note that for any random variable $Z$ and numbers $c \in (-\infty, \infty)$, $ \epsilon \in (0,1] $
%\begin{align}
%	\mathbb{E}[|Z + c|^{1 + \epsilon}] < \infty \Leftrightarrow  \mathbb{E}[|Z|^{1 + \epsilon}]. 
%\end{align}

\begin{lemma}[Variation of Lemma 1 in Bubeck et al, 2012]
	With probability at least $1 - \delta$,  
	\begin{align} 
		\left| m_t^{tr} (l) - \left< f \right>_l \right| \le 4 u^{\frac{1}{1 + \epsilon}} \left( \frac{\log (1/ \delta)}{n} \right)^{\frac{1}{1 + \epsilon}}. 
	\end{align}
\end{lemma}


\begin{proof}
	
	Consider the good event $\mathcal{G}_{t} := \left\{ f (A_i) - \left< f \right>_{L_t} \le \Psi, \quad i = 1,2, \cdots, t \right\}$. 
	In the following analysis, we focus our attention to where this event $\mathcal{G}_t$ is true. 
	
	By Proposition \ref{prop:cube-number}, we know $\left| \left< f \right>_{L_i} \right| \le \Psi$ for all $i$, as a consequence of the partition refinement rule. 
	
	Let $L_i$, $A_i$, $Y_i$ be the cube, arm and reward at round $i$. Then by Minkowski inequality, 
	\begin{align}
		\mathbb{E}_i \left| Y_i \right|^{1 + \epsilon} &=
		\mathbb{E}_i \left| Y_i - \left< f \right>_{L_i} + \left< f \right>_{L_i} \right|^{1 + \epsilon} \\
		&= \mathbb{E}_i |f(A_i) - \left< f \right>_{L_i} + \mathpzc{E}_{A_i} + \left< f \right>_{L_i} |^{1 + \epsilon}  \\
		&\le 2^{3 + 2\epsilon}  \Psi^{1 + \epsilon} + 2^{1 + \epsilon} u  
	\end{align} 
	 
	We first consider the case $n_t(l) > 0$, and let $ i_1, i_2, \cdots, i_{n_t(l)} $ be the times where $\mathbbm{1}[A_{i_j} \in l]$ ($j = 1,2,\cdots, n_{t (l)}$). We have the following: %$ Y_{i_j} = $
	\begin{align}
		\left| m_t^{tr} (l) - \left< f \right>_l \right| =& \left| \frac{\sum_{j = 1 }^{ n_t (l)  } Y_{i_j} \mathbbm{1}_{[|Y_{i_j}| \le B_j ]} }{ n_{t} (l) } - \left< f \right>_l \right| \\
%		=& \left| \frac{\sum_{i = 1 }^{ t - 1 } Y_i \mathbbm{1}_{[A_i \in l ]} \mathbbm{1}_{[|Y_i| \le B_i ]} }{ n_{t} (l) } - \left< f \right>_l \right| \\
		\le&  \left| \frac{ \sum_{j = 1 }^{ n_t (l)  } Y_{i_j} \mathbbm{1}_{[|Y_{i_j}| \le B_j ]} }{ n_{t} (l) } - \frac{ \sum_{j = 1 }^{ n_t(l) } \left< f \right>_l \mathbbm{1}_{[|Y_{i_j} | \le B_j ] } }{ n_{t} (l) } \right| \\
		&+ \left| \frac{ \sum_{j = 1 }^{ n_t(l) } \left( \left< f \right>_l \mathbbm{1}_{[|Y_{i_j} | \le B_j ] } - \left< f \right>_l \right) }{ n_{t} (l) } \right| \\ 
		=& \left| \frac{ \sum_{j = 1 }^{ n_t (l)  } Y_{i_j} \mathbbm{1}_{[|Y_{i_j}| \le B_j ]} }{ n_{t} (l) } - \frac{ \sum_{j = 1 }^{ n_t(l) } \left< f \right>_l \mathbbm{1}_{[|Y_{i_j} | \le B_j ] } }{ n_{t} (l) } \right| \\
		&+ \left| \frac{ \sum_{j = 1 }^{ n_t(l) } \left< f \right>_l \mathbbm{1}_{[|Y_{i_j} | > B_j ] }  }{ n_{t} (l) } \right| .
	\end{align}
	Since the sequence of random variables $\{ \left( Y_{i_j} - \left< f \right>_l \right) \mathbbm{1}_{[|Y_{i_j}| \le B_j ]} \}_j$ is a sub-sequence of $\{ \left( Y_{i} - \left< f \right>_l \right) \mathbbm{1}_{[|Y_{i_j}| \le B_j ]} \}_i$
\end{proof}



